Temporal Basis Function Models for Closed-Loop Neural Stimulation

Closed-loop neural stimulation provides novel therapies for neurological diseases such as Parkinson's disease (PD), but it is not yet clear whether artificial intelligence (AI) techniques can tailor closed-loop stimulation to individual patients or identify new therapies. Progress requires us to address a number of translational issues, including sample efficiency, training time, and minimizing loop latency such that stimulation may be shaped in response to changing brain activity. We propose temporal basis function models (TBFMs) to address these difficulties, and explore this approach in the context of excitatory optogenetic stimulation. We demonstrate the ability of TBF models to provide a single-trial, spatiotemporal forward prediction of the effect of optogenetic stimulation on local field potentials (LFPs) measured in two non-human primates. We further use simulations to demonstrate the use of TBF models for closed-loop stimulation, driving neural activity towards target patterns. The simplicity of TBF models allow them to be sample efficient, rapid to train (2-4min), and low latency (0.2ms) on desktop CPUs. We demonstrate the model on 40 sessions of previously published excitatory optogenetic stimulation data. For each session, the model required 15-20min of data collection to successfully model the remainder of the session. It achieved a prediction accuracy comparable to a baseline nonlinear dynamical systems model that requires hours to train, and superior accuracy to a linear state-space model. In our simulations, it also successfully allowed a closed-loop stimulator to control a neural circuit. Our approach begins to bridge the translational gap between complex AI-based approaches to modeling dynamical systems and the vision of using such forward prediction models to develop novel, clinically useful closed-loop stimulation protocols.

==> macro.tex <==
\usepackage{amsmath,amsfonts,amsthm,amssymb,amsopn,bm,mathtools}
\usepackage[margin=.9in]{geometry}
\usepackage{graphicx}
\usepackage{url}
\usepackage[hidelinks]{hyperref}
\usepackage[usenames,dvipsnames]{color}
\usepackage{fancyhdr}
\usepackage{multirow}
\usepackage{mdframed}
\usepackage{ifthen}

% calculus
% the differential operator
\makeatletter
\providecommand*{\diff}
{\@ifnextchar^{\DIfF}{\DIfF^{}}}
\def\DIfF^#1{
	\mathop{\mathrm{\mathstrut d}}
	\nolimits^{#1}\gobblespace}
\def\gobblespace{
	\futurelet\diffarg\opspace}
\def\opspace{
	\let\DiffSpace\!
	\ifx\diffarg(
	\let\DiffSpace\relax
	\else
	\ifx\diffarg[
	\let\DiffSpace\relax
	\else
	\ifx\diffarg\{
	\let\DiffSpace\relax
	\fi\fi\fi\DiffSpace}

\providecommand*{\pdiff}
{\@ifnextchar^{\pDIfF}{\pDIfF^{}}}
\def\pDIfF^#1{
	\mathop{\mathrm{\mathstrut \partial}}
	\nolimits^{#1}\gobblespace}
\def\gobblespace{
	\futurelet\diffarg\opspace}
\def\opspace{
	\let\DiffSpace\!
	\ifx\diffarg(
	\let\DiffSpace\relax
	\else
	\ifx\diffarg[
	\let\DiffSpace\relax
	\else
	\ifx\diffarg\{
	\let\DiffSpace\relax
	\fi\fi\fi\DiffSpace}

% derivative and partial derivative operators
\providecommand*{\deriv}[3][]{\frac{\diff^{#1}{#2}}{\diff {#3}^{#1}}}
\providecommand*{\pderiv}[3][]{\frac{\pdiff^{#1}{#2}}{\pdiff {#3}^{#1}}}
\providecommand*{\pderivcross}[3]{\frac{\pdiff^{2} {#1}}{\pdiff {#2} \pdiff {#3} }}

% set notation
\providecommand\given{}
\newcommand\SetSymbol[1][]{%
	\nonscript\:#1\vert
	\allowbreak
	\nonscript\:
	\mathopen{}}
\DeclarePairedDelimiterX\Set[1]\{\}{%
	\renewcommand\given{\SetSymbol[\delimsize]}
	#1
}
\newcommand{\set}[1]{\Set*{#1}}


% probability
\DeclarePairedDelimiterXPP\prob[1]{\mathop{\mathbb{P}}}{\lbrace}{\rbrace}{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
\newcommand{\Prob}[1]{\prob*{#1}}

\DeclarePairedDelimiterXPP\probability[2]{\mathop{\mathbb{P}}_{#1}}{\lbrace}{\rbrace}{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#2}
\newcommand{\Probability}[2]{\probability*{#1}{#2}}

\DeclarePairedDelimiterXPP\expectation[1]{\mathop{\mathbb{E}}}{\lbrack}{\rbrack}{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
\newcommand{\E}[1]{\expectation*{#1}}

\DeclarePairedDelimiterXPP\expectationdist[2]{\mathop{\mathbb{E}}_{#1}}{\lbrack}{\rbrack}{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#2}
\newcommand{\Exp}[2]{\expectationdist*{#1}{#2}}

\DeclarePairedDelimiterXPP\variance[1]{\mathop{\mathrm{Var}}}{\lbrack}{\rbrack}{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
\newcommand{\Var}[1]{\variance*{#1}}

\DeclarePairedDelimiterXPP\variancedist[2]{\mathop{\mathrm{Var}}_{#1}}{\lbrack}{\rbrack}{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#2}
\newcommand{\Variance}[2]{\variancedist*{#1}{#2}}

\DeclarePairedDelimiterXPP\covariance[2]{\mathop{\mathrm{Cov}}}{(}{)}{}{#1,\mathopen{}#2}
\newcommand{\Cov}[2]{\covariance*{#1}{#2}}


% Linear Algebra, symmetry notation
\newcommand{\Matrix}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\Tr}[1]{\mathop{\mathrm{Tr}}\squarebrack{#1}}

% norms
\DeclarePairedDelimiterXPP{\nrm}[2]{}{\lVert}{\rVert}{\ensuremath{_{#1}}}{\ifblank{#2}{\:\cdot\:}{#2}}
\newcommand{\norm}[2]{\nrm*{#1}{#2}}

\newcommand{\twonorm}[1]{\norm{2}{#1}}
\newcommand{\twonormsq}[1]{\norm{2}{#1}^2}
\newcommand{\opnorm}[1]{\norm{\mathrm{op}}{#1}}
\newcommand{\normF}[1]{\norm{\mathrm{F}}{#1}}


% parentheses
\DeclarePairedDelimiterX{\bracket}[3]{#1}{#2}{#3}

\newcommand{\abs}[1]{\bracket*{\lvert}{\rvert}{#1}}
\newcommand{\round}[1]{\bracket*{(}{)}{#1}}
\newcommand{\curly}[1]{\bracket*{\lbrace}{\rbrace}{#1}}
\newcommand{\squarebrack}[1]{\bracket*{\lbrack}{\rbrack}{#1}}

% For Convenience
\newcommand{\comment}[1]{\qquad\round{\text{#1}}}
\newcommand{\commentnewline}[1]{\qquad\qquad\qquad\qquad\qquad\qquad\comment{#1}\nonumber}
\newcommand{\inv}[1]{\frac{1}{#1}}
\newcommand{\sumi}[2]{\sum\limits_{i=#1}^{#2}}
\newcommand{\sumj}[2]{\sum\limits_{j=#1}^{#2}}
\newcommand{\sumk}[2]{\sum\limits_{k=#1}^{#2}}

\newcommand{\field}[1]{\mathbb{#1}}
\newcommand{\1}{\mathbf{1}}
\newcommand{\R}{\field{R}} % real domain
\newcommand{\bx}{\mathbf{x}}

% TODO command
\usepackage{xcolor}
\newcommand{\todo}{\textcolor{red!90!black}{\textbf{TODO}}}

\def\diag{\text{diag}}

%% operator in linear algebra, functional analysis
\newcommand{\inner}[2]{#1\cdot #2}
\renewcommand{\theenumi}{\alph{enumi}} 

\newcommand{\Perp}{\perp \! \! \! \perp}

\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\vct}[1]{\mathbf{#1}} % vector
\newcommand{\vect}[1]{\mathbf{#1}} % vector
\newcommand{\mat}[1]{\mathbf{#1}} % matrix
\newcommand{\cst}[1]{\mathsf{#1}} % constant
\newcommand{\points}[1]{\small\textcolor{magenta}{\emph{[#1 point\ifthenelse{\equal{#1}{1}}{}{s}]}} \normalsize}

% Define a new problem
\newcounter{aprob}
\newenvironment{aprob}[1][]{\refstepcounter{aprob}\par\medskip\noindent A\theaprob.#1 }

\newcounter{bprob}
\newenvironment{bprob}[1][]{\begin{mdframed} \refstepcounter{bprob}\par\medskip\noindent B\thebprob.#1 }
  {\vspace{1pt} \end{mdframed}}


\usepackage{listings}  % Include the listings-package
\lstset{language=Python}
\usepackage{float}
\usepackage{multicol}
\usepackage{enumitem}
\usepackage{wrapfig}

\def\P{\mathbb{P}}
\def\R{\mathbb{R}}

\newtheorem{lemma}{Lemma}

\DeclareMathOperator*{\argmax}{arg\,max} 
\DeclareMathOperator*{\argmin}{arg\,min} 
\global\long\def\dd{\textnormal{d}}

